MoVEInt: Mixture of Variational Experts for Learning Human-Robot Interactions from Demonstrations

Shared dynamics models are important for capturing the complexity and variability inherent in Human-Robot Interaction (HRI). Therefore, learning such shared dynamics models can enhance coordination and adaptability to enable successful reactive interactions with a human partner. In this work, we propose a novel approach for learning a shared latent space representation for HRIs from demonstrations in a Mixture of Experts fashion for reactively generating robot actions from human observations. We train a Variational Autoencoder (VAE) to learn robot motions regularized using an informative latent space prior that captures the multimodality of the human observations via a Mixture Density Network (MDN). We show how our formulation derives from a Gaussian Mixture Regression formulation that is typically used approaches for learning HRI from demonstrations such as using an HMM/GMM for learning a joint distribution over the actions of the human and the robot. We further incorporate an additional regularization to prevent "mode collapse", a common phenomenon when using latent space mixture models with VAEs. We find that our approach of using an informative MDN prior from human observations for a VAE generates more accurate robot motions compared to previous HMM-based or recurrent approaches of learning shared latent representations, which we validate on various HRI datasets involving interactions such as handshakes, fistbumps, waving, and handovers. Further experiments in a real-world human-to-robot handover scenario show the efficacy of our approach for generating successful interactions with four different human interaction partners.

==> hri-kobo-diff.tex <==

    \begin{figure*}[h!]
    \centering
    % \begin{subfigure}[b]{0.9\textwidth}
    %      \centering
             \includegraphics[width=0.18\textwidth]{img/kobo-recording/kobo-frame1.jpg}
        \includegraphics[width=0.18\textwidth]{img/kobo-recording/kobo-frame2.jpg}
        \includegraphics[width=0.18\textwidth]{img/kobo-recording/kobo-frame3.jpg}
        \includegraphics[width=0.18\textwidth]{img/kobo-recording/kobo-frame4.jpg}
        \includegraphics[width=0.18\textwidth]{img/kobo-recording/kobo-frame5.jpg}
        % \includegraphics[width=0.19\textwidth]{img/kobo-recording/kobo-rviz-frame1.png}
        % \includegraphics[width=0.19\textwidth]{img/kobo-recording/kobo-rviz-frame2.png}
        % \includegraphics[width=0.19\textwidth]{img/kobo-recording/kobo-rviz-frame3.png}
        % \includegraphics[width=0.19\textwidth]{img/kobo-recording/kobo-rviz-frame4.png}
        % \includegraphics[width=0.19\textwidth]{img/kobo-recording/kobo-rviz-frame5.png}
    % \end{subfigure} \\ 
    % \begin{subfigure}[b]{0.9\textwidth}
    %     \centering
    %     \includegraphics[width=0.19\textwidth,trim={0 5cm 0 10cm},clip]{img/pepper-recording/pepper-frame1.jpg}
    %     \includegraphics[width=0.19\textwidth,trim={0 5cm 0 10cm},clip]{img/pepper-recording/pepper-frame2.jpg}
    %     \includegraphics[width=0.19\textwidth,trim={0 5cm 0 10cm},clip]{img/pepper-recording/pepper-frame3.jpg}
    %     \includegraphics[width=0.19\textwidth,trim={0 5cm 0 10cm},clip]{img/pepper-recording/pepper-frame4.jpg}
    %     \includegraphics[width=0.19\textwidth,trim={0 5cm 0 10cm},clip]{img/pepper-recording/pepper-frame5.jpg} \\
    %     \includegraphics[width=0.19\textwidth,trim={8cm 0 0 0},clip]{img/pepper-recording/pepper-rviz-frame1.png}
    %     \includegraphics[width=0.19\textwidth,trim={8cm 0 0 0},clip]{img/pepper-recording/pepper-rviz-frame2.png}
    %     \includegraphics[width=0.19\textwidth,trim={8cm 0 0 0},clip]{img/pepper-recording/pepper-rviz-frame3.png}
    %     \includegraphics[width=0.19\textwidth,trim={8cm 0 0 0},clip]{img/pepper-recording/pepper-rviz-frame4.png}
    %     \includegraphics[width=0.19\textwidth,trim={8cm 0 0 0},clip]{img/pepper-recording/pepper-rviz-frame5.png}
    %     \caption{Rocket Fistbump Interaction with a Pepper robot.}
    %     \label{fig:pepper-fistbump}
    % \end{subfigure}

    \caption{Sample Human-Robot Interactions generated with the reactive motions generated by MoVEInt for a Bimanual Handover scenario.% (Red - Human observation, Dark Blue - Generated Robot Trajectory, Yellow, Purple, and Light Blue - MDN Components Decoded).
    }
    \label{fig:moveint-hri}
\end{figure*}


==> mse_table_diff.tex <==
\DIFaddbegin 

\DIFaddend \begin{table*}[h!]
    \centering
\vspace{2em}
% \resizebox{0.99\textwidth}{!}{
\begin{tabular}{|c|c|c|c|l|}
\hline
\DIFaddbeginFL 

\DIFaddendFL Dataset (units) & Action & MILD\DIFaddbeginFL \DIFaddFL{~\mbox{\cite{prasad2023learning} }\hskip0pt }\DIFaddendFL & B\"utepage et al.\DIFdelbeginFL \DIFdelFL{(2020) }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{~\mbox{\cite{butepage2020imitating} }\hskip0pt }\DIFaddendFL & \hfill \DIFdelbeginFL \DIFdelFL{LaMPInt }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{MoVEInt }\DIFaddendFL \hfill\\ \hline
\DIFdelbeginFL %DIFDELCMD < \multirow{4}{*}{\begin{tabular}{c}HHI\\(B\"utepage et al. 2020)\\(cm)\end{tabular}} %%%
\DIFdelendFL \DIFaddbeginFL \multirow{4}{*}{\begin{tabular}{c}HHI\\(B\"utepage et al.~\cite{butepage2020imitating})\\(cm)\end{tabular}} \DIFaddendFL & Hand Wave & 0.788 $\pm$ 1.226 &  4.121 $\pm$ 2.252 & \textbf{\DIFdelbeginFL \DIFdelFL{0.417 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.448 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.627}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.630}\DIFaddendFL } \\ \cline{2-5} 
& Handshake & 1.654 $\pm$ 1.549 &  1.181 $\pm$ 0.859 & \textbf{\DIFdelbeginFL \DIFdelFL{0.208 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.196 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.137}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.153}\DIFaddendFL }\\ \cline{2-5} 
& Rocket Fistbump & 0.370 $\pm$ 0.682 &  0.544 $\pm$ 1.249 & \textbf{\DIFdelbeginFL \DIFdelFL{0.116 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.123 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.191}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.175}\DIFaddendFL }\\ \cline{2-5} 
& Parachute Fistbump & 0.537 $\pm$ 0.579 &  0.977 $\pm$ 1.141 & \textbf{\DIFdelbeginFL \DIFdelFL{0.310 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.314 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.340}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.348}\DIFaddendFL } \\ \hline
\DIFdelbeginFL %DIFDELCMD < \multirow{4}{*}{\begin{tabular}{c}HRI-Pepper\\(B\"utepage et al. 2020)\\(rad)\end{tabular}} %%%
\DIFdelendFL \DIFaddbeginFL \multirow{4}{*}{\begin{tabular}{c}HRI-Pepper\\(B\"utepage et al.~\cite{butepage2020imitating})\\(rad)\end{tabular}} \DIFaddendFL & Hand Wave & 0.103 $\pm$ 0.103 & 0.664 $\pm$ 0.277 & \textbf{\DIFdelbeginFL \DIFdelFL{0.093 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.087 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.088}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.089}\DIFaddendFL }\\ \cline{2-5} 
 & Handshake & 0.056 $\pm$ 0.041 & 0.184 $\pm$ 0.141 & \textbf{\DIFdelbeginFL \DIFdelFL{0.016 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.015 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.013}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.014}\DIFaddendFL }\\ \cline{2-5} 
 & Rocket Fistbump & 0.018 $\pm$ 0.035 &  0.033 $\pm$ 0.045 & \textbf{0.007 $\pm$ \DIFdelbeginFL \DIFdelFL{0.014}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.015}\DIFaddendFL }\\ \cline{2-5} 
 & Parachute Fistbump & 0.088 $\pm$ 0.148 & 0.189 $\pm$ 0.196 & \textbf{\DIFdelbeginFL \DIFdelFL{0.056 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.048 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.127}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.112}\DIFaddendFL } \\ \hline
\DIFdelbeginFL %DIFDELCMD < \multirow{4}{*}{\begin{tabular}{c}HRI-Yumi\\(B\"utepage et al. 2020)\\(rad)\end{tabular}} %%%
\DIFdelendFL \DIFaddbeginFL \multirow{4}{*}{\begin{tabular}{c}HRI-Yumi\\(B\"utepage et al.~\cite{butepage2020imitating})\\(rad)\end{tabular}} \DIFaddendFL & Hand Wave & 1.033 $\pm$ 1.204 & \DIFdelbeginFL \textbf{\DIFdelFL{0.225 $\pm$ 0.302}} %DIFAUXCMD
%DIFDELCMD < & %%%
\DIFdelFL{0.408 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.225 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.369 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.302 }& \textbf{\DIFaddFL{0.147 $\pm$ 0.072}} \DIFaddendFL \\ \cline{2-5} 
 & Handshake & 0.068 $\pm$ 0.052 & 0.133 $\pm$ 0.214 & \textbf{\DIFdelbeginFL \DIFdelFL{0.066 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.057 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.034}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.044}\DIFaddendFL }\\ \cline{2-5} 
 & Rocket Fistbump & \DIFdelbeginFL \textbf{\DIFdelFL{0.128 $\pm$ 0.071}} %DIFAUXCMD
\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.128 $\pm$ 0.071 }\DIFaddendFL & 0.147 $\pm$ 0.119 & \DIFdelbeginFL \DIFdelFL{0.154 $\pm$ 0.074 }\DIFdelendFL \DIFaddbeginFL \textbf{\DIFaddFL{0.093 $\pm$ 0.045}} \DIFaddendFL \\ \cline{2-5} 
 & Parachute Fistbump & \textbf{0.028 $\pm$ 0.034} & 0.181 $\pm$ 0.155 & \DIFdelbeginFL \DIFdelFL{0.135 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.081 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.120}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.082}\DIFaddendFL \\ \hline
\DIFdelbeginFL %DIFDELCMD < \multirow{4}{*}{\begin{tabular}{c}HHI\\(NuiSI)\\(cm)\end{tabular}} %%%
\DIFdelendFL \DIFaddbeginFL \multirow{4}{*}{\begin{tabular}{c}HHI\\(NuiSI~\cite{prasad2023learning})\\(cm)\end{tabular}} \DIFaddendFL & Hand Wave & 0.408 $\pm$ 0.538 & 3.168 $\pm$ 3.392 & \textbf{\DIFdelbeginFL \DIFdelFL{0.270 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.298 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.284}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.274}\DIFaddendFL } \\ \cline{2-5} 
& Handshake & 0.311 $\pm$ 0.259 & 1.489 $\pm$ 3.327 & \textbf{\DIFdelbeginFL \DIFdelFL{0.165 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.149 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.102}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.120}\DIFaddendFL } \\ \cline{2-5} 
& Rocket Fistbump & 1.142 $\pm$ 1.375 & 3.576 $\pm$ 3.082 & \textbf{\DIFdelbeginFL \DIFdelFL{0.954 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.673 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.744}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.679}\DIFaddendFL } \\ \cline{2-5} 
& Parachute Fistbump & 0.453 $\pm$ 0.578 & 2.008 $\pm$ 2.024 & \textbf{\DIFdelbeginFL \DIFdelFL{0.328 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.291 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.348}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.199}\DIFaddendFL } \\ \hline
\DIFdelbeginFL %DIFDELCMD < \multirow{4}{*}{\begin{tabular}{c}HRI-Pepper\\(NuiSI)\\(rad)\end{tabular}} %%%
\DIFdelendFL \DIFaddbeginFL \multirow{4}{*}{\begin{tabular}{c}HRI-Pepper\\(NuiSI~\cite{prasad2023learning})\\(rad)\end{tabular}} \DIFaddendFL & Hand Wave & 0.046 $\pm$ 0.059 & 0.057 $\pm$ 0.093 & \textbf{\DIFdelbeginFL \DIFdelFL{0.038 $\pm$ }\DIFdelendFL 0.044 \DIFaddbeginFL \DIFaddFL{$\pm$ 0.048}\DIFaddendFL } \\ \cline{2-5} 
& Handshake & 0.020 $\pm$ 0.014 & 0.083 $\pm$ 0.075 & \textbf{\DIFdelbeginFL \DIFdelFL{0.012 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.011 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.010}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.008}\DIFaddendFL } \\ \cline{2-5} 
& Rocket Fistbump  & 0.077 $\pm$ 0.067 & 0.101 $\pm$ 0.086 & \textbf{\DIFdelbeginFL \DIFdelFL{0.054 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.045 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.053}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.045}\DIFaddendFL } \\ \cline{2-5} 
& Parachute Fistbump & 0.022 $\pm$ 0.027 & 0.049 $\pm$ 0.040 & \textbf{\DIFdelbeginFL \DIFdelFL{0.019 }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.017 }\DIFaddendFL $\pm$ \DIFdelbeginFL \DIFdelFL{0.024}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{0.014}\DIFaddendFL } \\ \hline
HHI-Handovers & Unimanual & 0.441 $\pm$ 0.280 & 1.133 $\pm$ 0.721 & \textbf{0.441 $\pm$ 0.221}\\ \cline{2-5} 
(Kshirsagar et al.\DIFdelbeginFL \DIFdelFL{2023}\DIFdelendFL \DIFaddbeginFL \DIFaddFL{~\mbox{\cite{kshirsagar2023dataset}}\hskip0pt }\DIFaddendFL ) (cm) & Bimanual & 0.869 $\pm$ 0.964 & 0.990 $\pm$ 0.764 & \textbf{0.685 $\pm$ 0.643} \\ \hline

\end{tabular}
% }
\vspace{0.5em}
    \caption{Prediction MSE for robot trajectories after observing the human partner averaged over all joints and timesteps. Results for the HHI scenarios are in cm and for the HRI scenarios are in radians. (Lower is better)}
    \label{tab:pred_mse}
\vspace{-1em}
\end{table*}
